Biomedical image analysis competitions: The state of current participation practice

The number of international benchmarking competitions is steadily increasing in various fields of machine learning (ML) research and practice. So far, however, little is known about the common practice as well as bottlenecks faced by the community in tackling the research questions posed. To shed light on the status quo of algorithm development in the specific field of biomedical imaging analysis, we designed an international survey that was issued to all participants of challenges conducted in conjunction with the IEEE ISBI 2021 and MICCAI 2021 conferences (80 competitions in total). The survey covered participants' expertise and working environments, their chosen strategies, as well as algorithm characteristics. A median of 72% challenge participants took part in the survey. According to our results, knowledge exchange was the primary incentive (70%) for participation, while the reception of prize money played only a minor role (16%). While a median of 80 working hours was spent on method development, a large portion of participants stated that they did not have enough time for method development (32%). 25% perceived the infrastructure to be a bottleneck. Overall, 94% of all solutions were deep learning-based. Of these, 84% were based on standard architectures. 43% of the respondents reported that the data samples (e.g., images) were too large to be processed at once. This was most commonly addressed by patch-based training (69%), downsampling (37%), and solving 3D analysis tasks as a series of 2D tasks. K-fold cross-validation on the training set was performed by only 37% of the participants and only 50% of the participants performed ensembling based on multiple identical models (61%) or heterogeneous models (39%). 48% of the respondents applied postprocessing steps.

==> authors.tex <==
% Please DON'T touch the authors here!!!
% This is automatically generated from an Excel file.
% Tell Matze if you want to edit.

\author{Lena Maier-Hein}
\email{l.maier-hein@dkfz-heidelberg.de}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Matthias Eisenmann}
\email{m.eisenmann@dkz-heidelberg.de}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Annika Reinke}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Annette Kopp-Schneider}
\affiliation{%
 \institution{Division of Biostatistics, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Vivienn Weru}
\affiliation{%
 \institution{Division of Biostatistics, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Klaus Maier-Hein}
\affiliation{%
 \institution{Division of Medical Image Computing, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Fabian Isensee}
\affiliation{%
 \institution{Applied Computer Vision Lab, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Paul Jäger}
\affiliation{%
 \institution{Interactive Machine Learning, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Patrick Godau}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Tim Adler}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Minu Dietlinde Tizabi}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Amine Yamlahi}
\affiliation{%
 \institution{Division of Intelligent Medical Systems, German Cancer Research Center, Heidelberg}
 \country{Germany}
}

\author{Veronika Cheplygina}
\affiliation{%
 \institution{ITU Copenhagen}
 \country{Denmark}
}

\author{Michal Kozubek}
\affiliation{%
 \institution{Masaryk University}
 \country{Czech Republic}
}

\author{Carlos Ortiz de Solórzano}
\affiliation{%
 \institution{Center for Applied Medical Research, Pamplona}
 \country{Spain}
}

\author{Donglai  Wei}
\affiliation{%
 \institution{School of Engineering and Applied Science, Harvard University}
 \country{USA}
}

\author{Sharib Ali}
\affiliation{%
 \institution{Department of Engineering Science, Big Data Institute, University of Oxford}
 \country{UK}
}

\author{Samiksha  Pachade}
\affiliation{%
 \institution{Shri Guru Gobind Singhji Institute of Engineering and Technology, Nanded, Maharashtra}
 \country{India}
}

\author{Anubha  Gupta}
\affiliation{%
 \institution{SBILab, Department of ECE, IIIT-Delhi}
 \country{India}
}

\author{Alison  Noble}
\affiliation{%
 \institution{Institute of Biomedical Engineering, University of Oxford}
 \country{UK}
}

\author{Elizabeth  Wilden}
\affiliation{%
 \institution{Institute of Biomedical Engineering, University of Oxford}
 \country{UK}
}

\author{Zhengbo Luo}
\affiliation{%
 \institution{Waseda University}
 \country{Japan}
}

\author{Tim Scherr}
\affiliation{%
 \institution{Karlsruhe Institute of Technology}
 \country{Germany}
}

\author{Dominik Müller}
\affiliation{%
 \institution{IT-Infrastrukturen für die Translationale Medizinische Forschung, Universität Augsburg}
 \country{Germany}
}

\author{Haoyu Wang}
\affiliation{%
 \institution{Shanghai Jiao Tong University}
 \country{China}
}

\author{Xin Zhao}
\affiliation{%
 \institution{The Center for Research on Intelligent System and Engineering, Institute of Automation, Chinese Academy of Sciences}
 \country{China}
}

\author{Young-tack Oh}
\affiliation{%
 \institution{Sungkyunkwan University, Suwon}
 \country{Korea}
}

\author{Hung Yeh}
\affiliation{%
 \institution{National United University}
 \country{nan}
}

\author{Tianqi Guo}
\affiliation{%
 \institution{Purdue University}
 \country{nan}
}

\author{Yangyang Wang}
\affiliation{%
 \institution{University of Missouri-Columbia}
 \country{USA}
}

\author{Edward Ho}
\affiliation{%
 \institution{Schulich School of Medicine \& Dentistry, Western University}
 \country{Canada}
}

\author{Filip Lux}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Oleh Dzyubachyk}
\affiliation{%
 \institution{nan}
 \country{The Netherlands}
}

\author{Andrew Cohen}
\affiliation{%
 \institution{Drexel University}
 \country{nan}
}

\author{Sokratis Makrogiannis}
\affiliation{%
 \institution{Delaware State University}
 \country{nan}
}

\author{Xinliang Wang}
\affiliation{%
 \institution{Beihang University}
 \country{China}
}

\author{Rina Bao}
\affiliation{%
 \institution{University of Missouri-Columbia}
 \country{USA}
}

\author{Constantin Pape}
\affiliation{%
 \institution{EMBL Heidelberg}
 \country{Germany}
}

\author{Tianyuan Gan}
\affiliation{%
 \institution{College of Biomedical Engineering and Instrument Science, Zhejiang University}
 \country{China}
}

\author{Gorkem Polat}
\affiliation{%
 \institution{Middle East Technical University}
 \country{nan}
}

\author{Ikbeom Jang}
\affiliation{%
 \institution{Massachusetts General Hospital}
 \country{USA}
}

\author{yan zeng}
\affiliation{%
 \institution{Beijing University of Technology, Beijing}
 \country{China}
}

\author{Kele Xu}
\affiliation{%
 \institution{National University of Defense Technology}
 \country{nan}
}

\author{Doyeob Yeo}
\affiliation{%
 \institution{Electronics and Telecommunications Research Institute}
 \country{nan}
}

\author{Kele Xu}
\affiliation{%
 \institution{National University of Defense Technology}
 \country{nan}
}

\author{Zhili Li}
\affiliation{%
 \institution{University of Science and Technology of China}
 \country{China}
}

\author{Adrian Galdran}
\affiliation{%
 \institution{Bournemouth University}
 \country{nan}
}

\author{Yixuan Yuan}
\affiliation{%
 \institution{City University of Hong Kong}
 \country{Hong Kong}
}

\author{Vajira Thambawita}
\affiliation{%
 \institution{SimulaMet}
 \country{Norway}
}

\author{Pradyumna Gupta}
\affiliation{%
 \institution{Indian Institute of Technology (Indian School of Mines), Dhanbad}
 \country{India}
}

\author{Mahmood Haithami}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Eason Wong}
\affiliation{%
 \institution{CUHK}
 \country{Hong Kong}
}

\author{Nicholas  Heller}
\affiliation{%
 \institution{University of Minnesota Robotics Institute (MnRI)}
 \country{USA}
}

\author{Melanie Ganz}
\affiliation{%
 \institution{Neurobiology Research Unit, Copenhagen University Hospital, Rigshospitalet, Copenhagen}
 \country{Denmark}
}

\author{Hannah Eichhorn}
\affiliation{%
 \institution{Neurobiology Research Unit, Copenhagen University Hospital, Rigshospitalet, Copenhagen}
 \country{Denmark}
}

\author{Reuben Dorent}
\affiliation{%
 \institution{King’s College London}
 \country{UK}
}

\author{Tom Vercauteren}
\affiliation{%
 \institution{King’s College London}
 \country{UK}
}

\author{Sandy Engelhardt}
\affiliation{%
 \institution{Working Group "Artificial Intelligence in Cardiovascular Medicine" (AICM), University Hospital Heidelberg}
 \country{Germany}
}

\author{Moi Hoon Yap}
\affiliation{%
 \institution{Human-Centred Computing; Manchester Metropolitan University}
 \country{UK}
}

\author{Sebastian Bodenstedt}
\affiliation{%
 \institution{Translational Surgical Oncology - National Center for Tumor Diseases (NCT), Partner Site Dresden, Fetscherstraße 74, PF 64, 01307 Dresden}
 \country{Germany}
}

\author{Jorge  Bernal}
\affiliation{%
 \institution{Universitat Autònoma de Barcelona \& Computer Vision Center}
 \country{Spain}
}

\author{Chinedu Innocent Nwoye}
\affiliation{%
 \institution{ICube, University of Strasbourg}
 \country{France}
}

\author{Deepak Alapatt}
\affiliation{%
 \institution{ICube, University of Strasbourg}
 \country{France}
}

\author{Armine Vardazaryan}
\affiliation{%
 \institution{IHU Strasbourg}
 \country{France}
}

\author{Nicolas Padoy}
\affiliation{%
 \institution{ICube, University of Strasbourg, France; IHU Strasbourg}
 \country{France}
}

\author{Sophia Bano}
\affiliation{%
 \institution{Wellcome/EPSRC Centre for Interventional and Surgical Sciences, University College London, London}
 \country{UK}
}

\author{Arnaud Huaulmé}
\affiliation{%
 \institution{Univ Rennes, INSERM, LTSI - UMR 1099, F35000, Rennes}
 \country{France}
}

\author{Aneeq Zia}
\affiliation{%
 \institution{Intuitive Surgical Inc}
 \country{USA}
}

\author{Gabriel Girard}
\affiliation{%
 \institution{CIBM Center for Biomedical Imaging \& Centre Hospitalier Universitaire Vaudois \& École Polytechnique Fédérale de Lausanne}
 \country{Switzerland}
}

\author{Jun Ma}
\affiliation{%
 \institution{Nanjing University of Science and Technology}
 \country{China}
}

\author{Spyridon Bakas}
\affiliation{%
 \institution{Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA}
 \country{USA}
}

\author{Sarthak Pati}
\affiliation{%
 \institution{Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA}
 \country{USA}
}

\author{Maximilian Zenk}
\affiliation{%
 \institution{Medical Image Computing, German Cancer Research Center (DKFZ), Heidelberg}
 \country{Germany}
}

\author{Kelly Payette}
\affiliation{%
 \institution{Kelly Payette, University of Zurich and University Children's Hospital Zurich}
 \country{Switzerland}
}

\author{Adrien Depeursinge}
\affiliation{%
 \institution{Institute of Information Systems, University of Applied Sciences and Arts Western Switzerland (HES-SO); Lausanne University Hospital (CHUV)}
 \country{Switzerland}
}

\author{Vincent Andrearczyk}
\affiliation{%
 \institution{University of Applied Sciences and Arts Western Switzerland (HES-SO)}
 \country{Switzerland}
}

\author{Valentin Oreiller}
\affiliation{%
 \institution{University of Applied Sciences and Arts Western Switzerland (HES-SO)}
 \country{Switzerland}
}

\author{Mattias Heinrich}
\affiliation{%
 \institution{University of Lübeck}
 \country{Germany}
}

\author{David Zimmerer}
\affiliation{%
 \institution{Medical Image Computing, German Cancer Research Center (DKFZ), Heidelberg}
 \country{Germany}
}

\author{Marc Aubreville}
\affiliation{%
 \institution{Technische Hochschule Ingolstadt}
 \country{Germany}
}

\author{Carlos Martín-Isla}
\affiliation{%
 \institution{Universitat de Barcelona}
 \country{Spain}
}

\author{Bjoern Menze}
\affiliation{%
 \institution{University of Zuerich, Switzerland; Technical University of Munich}
 \country{Germany}
}

\author{Hongwei Bran Li}
\affiliation{%
 \institution{University of Zuerich, Switzerland; Technical University of Munich}
 \country{Germany}
}

\author{Ujjwal Baid}
\affiliation{%
 \institution{Center for Biomedical Image Computing and Analytics (CBICA), University of Pennsylvania, Philadelphia, PA}
 \country{USA}
}

\author{Vivek Singh Bawa}
\affiliation{%
 \institution{Visual Artificial Intelligence Lab, Oxford Brookes University, Oxford}
 \country{UK}
}

\author{Jianning Li}
\affiliation{%
 \institution{Graz University of Technology \& Medical University of Graz}
 \country{Austria}
}

\author{Jan Egger}
\affiliation{%
 \institution{Graz University of Technology \& Medical University of Graz}
 \country{Austria}
}

\author{Carole Sudre}
\affiliation{%
 \institution{MRC Unit for Lifelong Health and Ageing, University College London, UK; Centre for Medical Image Computing, University College London, UK; School of Biomedical Engineering \& Imaging Sciences, King's College London, UK; Dementia Research Centre, University College London}
 \country{UK}
}

\author{Kimberlin van Wijnen}
\affiliation{%
 \institution{Biomedical Imaging Group, Erasmus MC}
 \country{The Netherlands}
}

\author{Niranjan Balu}
\affiliation{%
 \institution{Department of Radiology, University of Washington}
 \country{USA}
}

\author{Chun Yuan}
\affiliation{%
 \institution{Department of Radiology, University of Washington}
 \country{USA}
}

\author{Chuanbo Wang}
\affiliation{%
 \institution{Big Data Analytics and Visualization Laboratory, University of Wisconsin at Milwaukee, Milwaukee, 3200 N. Cramer St, Milwaukee, WI 53211}
 \country{USA}
}

\author{Zeyun Yu}
\affiliation{%
 \institution{Big Data Analytics and Visualization Laboratory, University of Wisconsin at Milwaukee, Milwaukee, 3200 N. Cramer St, Milwaukee, WI 53211}
 \country{USA}
}

\author{Olivier Commowick}
\affiliation{%
 \institution{INRIA Rennes - Bretagne Atlantique, Empenn research team, Campus de Beaulieu, 35000 Rennes}
 \country{France}
}

\author{Jinwook Choi}
\affiliation{%
 \institution{Seoul National University Hospital, Seoul}
 \country{South Korea}
}

\author{Hyunjeong Kim}
\affiliation{%
 \institution{Seoul National University Hospital, Seoul}
 \country{South Korea}
}

\author{Heonjin Ha}
\affiliation{%
 \institution{Saige Research}
 \country{nan}
}

\author{Zhiwei Chen}
\affiliation{%
 \institution{SHAANXI NORMAL UNIVERSITY}
 \country{nan}
}

\author{Yi Lv}
\affiliation{%
 \institution{Beihang University}
 \country{China}
}

\author{Ruize Shi}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Zhiqiang Shen}
\affiliation{%
 \institution{Fuzhou University}
 \country{China}
}

\author{Jimin Heo}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Lena Philipp}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Niklas Agethen}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Timo Günnemann}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Felix Thielke}
\affiliation{%
 \institution{University of Bremen; Fraunhofer MEVIS}
 \country{Germany}
}

\author{Hans Meine}
\affiliation{%
 \institution{University of Bremen; Fraunhofer MEVIS}
 \country{Germany}
}

\author{Jannes Adam}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Robert Bohnsack}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{René Finzel}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Marcel Plutat}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Markus Rink}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Tingting Xue}
\affiliation{%
 \institution{University of Bremen}
 \country{Germany}
}

\author{Vivek Pawar}
\affiliation{%
 \institution{Endimension Tech.}
 \country{nan}
}

\author{Christina B. Lund}
\affiliation{%
 \institution{Image Sciences Institute, UMC Utrecht, Utrecht University}
 \country{nan}
}

\author{Matej Gazda}
\affiliation{%
 \institution{Technical University of Kosice}
 \country{nan}
}

\author{Lizhan Xu}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Jianhui Wen}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Timothy Kline}
\affiliation{%
 \institution{Mayo Clinic}
 \country{nan}
}

\author{Abhi Lad}
\affiliation{%
 \institution{Pandit Deendayal Energy University}
 \country{nan}
}

\author{Sajan Gohil}
\affiliation{%
 \institution{Pandit Deendayal Energy University}
 \country{nan}
}

\author{Alex Golts}
\affiliation{%
 \institution{IBM Research}
 \country{nan}
}

\author{Chaonan Lin}
\affiliation{%
 \institution{Fuzhou University}
 \country{nan}
}

\author{Zhongchen Zhao}
\affiliation{%
 \institution{Shanghai Jiao Tong university}
 \country{nan}
}

\author{Jianpeng Zhang}
\affiliation{%
 \institution{Northwestern Polytechnical University}
 \country{China}
}

\author{Tian He}
\affiliation{%
 \institution{Fuzhou University}
 \country{nan}
}

\author{Kevin Blansit}
\affiliation{%
 \institution{Subtle Medical}
 \country{nan}
}

\author{Di Fan}
\affiliation{%
 \institution{University of California, Irvine}
 \country{nan}
}

\author{Chen Xiaofei}
\affiliation{%
 \institution{Southeast University}
 \country{nan}
}

\author{Maria  Baldeon Calisto }
\affiliation{%
 \institution{Universidad San Francisco de Quito }
 \country{nan}
}

\author{Hao Li}
\affiliation{%
 \institution{Vanderbilt University}
 \country{nan}
}

\author{Kai Yao}
\affiliation{%
 \institution{School of Advanced Technology, Xi’an Jiaotong-Liverpool University}
 \country{China}
}

\author{Han Liu}
\affiliation{%
 \institution{Vanderbilt University, Nashville, Tennessee}
 \country{USA}
}

\author{Smriti Joshi}
\affiliation{%
 \institution{University of Barcelona}
 \country{Spain}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{Huifeng Yao}
\affiliation{%
 \institution{Shandong University}
 \country{nan}
}

\author{Jiacheng Wang}
\affiliation{%
 \institution{Xiamen University}
 \country{nan}
}

\author{Yusely Ruiz-Gonzalez}
\affiliation{%
 \institution{Universidad Central "Marta Abreu" de Las Villas}
 \country{nan}
}

\author{Salman Ahmed}
\affiliation{%
 \institution{National University of Computer and Emerging Sciences, Islamabad}
 \country{nan}
}

\author{Hammad Naveed}
\affiliation{%
 \institution{National University of Computer and Emerging Sciences, Islamabad}
 \country{nan}
}

\author{Alfonso Medela}
\affiliation{%
 \institution{Legit Health}
 \country{nan}
}

\author{Adrian Galdran}
\affiliation{%
 \institution{Bournemouth University}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{Post-doc Researcher at École Nationale d'Ingénieurs de Brest, France}
 \country{nan}
}

\author{Chuantao Xie Chuantao Xie}
\affiliation{%
 \institution{Shanghai University}
 \country{nan}
}

\author{SUJIT KUMAR DAS}
\affiliation{%
 \institution{Department of Computer Science and Engineering, National Institute of Technology Silchar, India}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{postdoc}
 \country{nan}
}

\author{Arnab Mishra}
\affiliation{%
 \institution{Department of Computer Science and Engineering, National Institute of Technology Silchar, India}
 \country{nan}
}

\author{Fuyuan Liao}
\affiliation{%
 \institution{Xi'an Technological Unoversity, China}
 \country{nan}
}

\author{Louise Bloch}
\affiliation{%
 \institution{Department of Computer Science, University of Applied Sciences and Arts Dortmund, Dortmund, Germany; Institute for Medical Informatics, Biometry and Epidemiology (IMIBE), University Hospital Essen, Essen, Germany}
 \country{nan}
}

\author{Christoph M. Friedrich}
\affiliation{%
 \institution{Department of Computer Science, University of Applied Sciences and Arts Dortmund, Dortmund, Germany; Institute for Medical Informatics, Biometry and Epidemiology (IMIBE), University Hospital Essen, Essen, Germany }
 \country{nan}
}

\author{Raphael Brüngel}
\affiliation{%
 \institution{Department of Computer Science, University of Applied Sciences and Arts Dortmund, Dortmund, Germany; Institute for Medical Informatics, Biometry and Epidemiology (IMIBE), University Hospital Essen, Essen, Germany}
 \country{nan}
}

\author{Orhun Güley}
\affiliation{%
 \institution{Master's student}
 \country{nan}
}

\author{Wolfgang Reiter}
\affiliation{%
 \institution{Wintegral GmbH}
 \country{nan}
}

\author{Bruno Oliveira}
\affiliation{%
 \institution{2Ai – School of Technology, IPCA, Barcelos, Portugal}
 \country{nan}
}

\author{Nuno R. Freitas}
\affiliation{%
 \institution{CMEMS-Uminho, University of Minho, Portugal}
 \country{nan}
}

\author{Sylvain Guy}
\affiliation{%
 \institution{GMCAO/CAMI team at TIMC Lab UMR 5525 CNRS, UGA, Grenoble France}
 \country{nan}
}

\author{Sandrine Voros}
\affiliation{%
 \institution{GMCAO/CAMI team at TIMC Lab UMR 5525 CNRS, UGA, Grenoble France}
 \country{nan}
}

\author{Jonathan Zamora-Anaya}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Shunkai Yu}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Yuheng Zhi}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Jingpei Lu}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Shan Lin}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Michael Yip}
\affiliation{%
 \institution{University of California San Diego}
 \country{nan}
}

\author{Baosheng Zou}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{SeulGi Hong}
\affiliation{%
 \institution{VisionAI, hutom}
 \country{nan}
}

\author{SeungBum Hong }
\affiliation{%
 \institution{VisionAI, hutom }
 \country{nan}
}

\author{Min-Kook  Choi }
\affiliation{%
 \institution{VisionAI, hutom}
 \country{nan}
}

\author{Seungbum Hong}
\affiliation{%
 \institution{VisionAI, hutom}
 \country{nan}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{David Owen}
\affiliation{%
 \institution{Digital Surgery, Medtronic}
 \country{nan}
}

\author{Abdolrahim Kadkhodamohammadi}
\affiliation{%
 \institution{Digital Surgery, Medtronic}
 \country{nan}
}

\author{Maria Grammatikopoulou}
\affiliation{%
 \institution{Digital Surgery, Medtronic}
 \country{nan}
}

\author{Imanol Luengo}
\affiliation{%
 \institution{Digital Surgery, Medtronic}
 \country{nan}
}

\author{Danail Stoyanov}
\affiliation{%
 \institution{Digital Surgery, Medtronic; University College London}
 \country{nan}
}

\author{Junwen Pan}
\affiliation{%
 \institution{Tianjin University}
 \country{nan}
}

\author{Cheng Bian}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Adrian Krenzer}
\affiliation{%
 \institution{University of Würzburg}
 \country{nan}
}

\author{Tianqi XIANG}
\affiliation{%
 \institution{The Hong Kong University of Science and Technology}
 \country{nan}
}

\author{Amine Yamlahi}
\affiliation{%
 \institution{Intelligent Medical Systems, German Cancer Research Center, Heidelberg, Germany}
 \country{nan}
}

\author{Rong Tao}
\affiliation{%
 \institution{Institute of Medical Robotics, Shanghai Jiao Tong University}
 \country{nan}
}

\author{Raviteja Sista}
\affiliation{%
 \institution{Centre of Excellence in Artificial Intelligence, Indian Institute of Technology Kharagpur}
 \country{nan}
}

\author{jiacheng wang}
\affiliation{%
 \institution{xiamen university}
 \country{nan}
}

\author{Ling Li}
\affiliation{%
 \institution{School of Management, Hefei University of Technology, Hefei, China}
 \country{nan}
}

\author{Bokai Zhang}
\affiliation{%
 \institution{Johnson \& Johnson}
 \country{nan}
}

\author{Fangfang Xia}
\affiliation{%
 \institution{University of Chicago}
 \country{nan}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{Yuxuan Yang}
\affiliation{%
 \institution{School of Management, Hefei University of Technology}
 \country{nan}
}

\author{Bruno Oliveira}
\affiliation{%
 \institution{2Ai - School of Technology, IPCA, Barcelos, Portugal}
 \country{nan}
}

\author{Finn Gaida}
\affiliation{%
 \institution{Technical University Munich}
 \country{nan}
}

\author{Deepak Alapatt}
\affiliation{%
 \institution{University of Strasbourg}
 \country{nan}
}

\author{Ricardo Sanchez-Matilla}
\affiliation{%
 \institution{Digital Surgerya Medtronic Company}
 \country{nan}
}

\author{Julian Abbing}
\affiliation{%
 \institution{University of Twente; Johnson and Johnson}
 \country{nan}
}

\author{Beerend Gerats}
\affiliation{%
 \institution{University of Twente}
 \country{nan}
}

\author{Neil Getty}
\affiliation{%
 \institution{Government Research}
 \country{nan}
}

\author{Yueming Jin}
\affiliation{%
 \institution{University College London}
 \country{nan}
}

\author{Winnie Pang}
\affiliation{%
 \institution{National University of Singapore}
 \country{nan}
}

\author{Szymon Plotka}
\affiliation{%
 \institution{Sano Centre for Computational Medicine, Cracow, Poland}
 \country{nan}
}

\author{Rishab Khantwal}
\affiliation{%
 \institution{Student at Indian Institute of Technology Bombay}
 \country{nan}
}

\author{Chiara Lena}
\affiliation{%
 \institution{Politecnico di Milano}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{postdoc researcher}
 \country{nan}
}

\author{Bogyu Park}
\affiliation{%
 \institution{Hutom Inc. (Develop AI Surgical Platform) }
 \country{nan}
}

\author{Yunshuang Li}
\affiliation{%
 \institution{Zhejiang University}
 \country{nan}
}

\author{Michael Peven}
\affiliation{%
 \institution{Johns Hopkins University}
 \country{nan}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{Quang-Minh Nguyen}
\affiliation{%
 \institution{Laboratoire du Traitement du Signal et de l'Image - INSERM UMR 1099}
 \country{nan}
}

\author{SATYADWYOOM KUMAR}
\affiliation{%
 \institution{Bachelor of Engineering}
 \country{nan}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{Sara Bosticardo}
\affiliation{%
 \institution{University of Verona}
 \country{nan}
}

\author{Dogu Baran Aydogan}
\affiliation{%
 \institution{University of Eastern Finland}
 \country{nan}
}

\author{Kurt Schilling}
\affiliation{%
 \institution{Vanderbilt University Medical Center}
 \country{nan}
}

\author{Ye Wu}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Nagesh Adluru}
\affiliation{%
 \institution{University of Wisconsin, Madison}
 \country{nan}
}

\author{Patryk Filipiak}
\affiliation{%
 \institution{Center for Advanced Imaging Innovation and Research (CAI2R), Department of Radiology, NYU Langone Health, New York, NY, USA}
 \country{nan}
}

\author{Sina Mansour L.}
\affiliation{%
 \institution{Department of Biomedical Engineering, The University of Melbourne, Parkville, Victoria, Australia}
 \country{nan}
}

\author{Tomasz Pieciak}
\affiliation{%
 \institution{AGH University of Science and Technology, Kraków, Poland;  Universidad de Valladolid, Valladolid, Spain}
 \country{nan}
}

\author{Alberto Cacciola}
\affiliation{%
 \institution{Brain Mapping Lab, Department of Biomedical, Dental Sciences and Morphological and Functional Images, University of Messina, Messina, Italy}
 \country{nan}
}

\author{Kenji Marshall}
\affiliation{%
 \institution{McGill University}
 \country{nan}
}

\author{Antoine Théberge}
\affiliation{%
 \institution{Université de Sherbrooke}
 \country{nan}
}

\author{Doohee Lee}
\affiliation{%
 \institution{MEDICALIP Co., Ltd.}
 \country{nan}
}

\author{YiFei Wang}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Rian Huang}
\affiliation{%
 \institution{National-Regional Key Technology Engineering Laboratory for Medical Ultrasound, Guangdong Key Laboratory for Biomedical Measurements and Ultrasound Imaging, School of Biomedical Engineering, Health Science Center, Shenzhen University, Shenzhen, China}
 \country{nan}
}

\author{Xue Feng}
\affiliation{%
 \institution{University of Virginia}
 \country{nan}
}

\author{Ziqi Zhou}
\affiliation{%
 \institution{Shenzhen university}
 \country{nan}
}

\author{Cuong Nguyen Quoc}
\affiliation{%
 \institution{University of Information Technology, Vietnam National University Ho Chi Minh City}
 \country{nan}
}

\author{Edward Henderson}
\affiliation{%
 \institution{The University of Manchester}
 \country{nan}
}

\author{Ziyan Huang}
\affiliation{%
 \institution{Shanghai Jiao Tong University}
 \country{nan}
}

\author{Talha Anwar}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{postdoc reseacher}
 \country{nan}
}

\author{Franz Thaler}
\affiliation{%
 \institution{Institute of Computer Vision and Graphics, Graz University of Technology; Gottfried Schatz Research Center: Biophysics, Medical University of Graz}
 \country{nan}
}

\author{Jiapeng Zhang}
\affiliation{%
 \institution{University of Shanghai for Science and Technology}
 \country{nan}
}

\author{Yuanhong Jiang}
\affiliation{%
 \institution{Shanghai Jiao Tong University}
 \country{nan}
}

\author{Fan Zhang}
\affiliation{%
 \institution{Fosun Aitrox information technology Ltd.}
 \country{nan}
}

\author{Akis Linardos}
\affiliation{%
 \institution{I'm a PhD student at the University of Barcelona}
 \country{nan}
}

\author{Muhammad Irfan Khan}
\affiliation{%
 \institution{Turku University of Applied Sciences}
 \country{nan}
}

\author{Leon Maechler}
\affiliation{%
 \institution{ENS Paris}
 \country{nan}
}

\author{Ece Isik Polat}
\affiliation{%
 \institution{Research Assistant}
 \country{nan}
}

\author{Sahil Nalawade}
\affiliation{%
 \institution{UT Southwestern Medical Center}
 \country{nan}
}

\author{Kamlesh Pawar}
\affiliation{%
 \institution{Monash University}
 \country{nan}
}

\author{Davood Karimi}
\affiliation{%
 \institution{Harvard Medical School}
 \country{nan}
}

\author{Lucas Fidon}
\affiliation{%
 \institution{School of Biomedical Engineering \& Imaging Sciences}
 \country{nan}
}

\author{Bella Specktor Fadida}
\affiliation{%
 \institution{Hebrew University of Jerusalem}
 \country{nan}
}

\author{Netanell Avisdris}
\affiliation{%
 \institution{School of Computer Science and Engineering, Hebrew University of Jerusalem, Israel; Sagol Brain Institute, Tel Aviv Sourasky Medical Center, Israel}
 \country{nan}
}

\author{Yi Lv}
\affiliation{%
 \institution{Beijing Institute of Technology}
 \country{nan}
}

\author{Daniel Sobotka}
\affiliation{%
 \institution{Computational Imaging Research Lab, Department of Biomedical Imaging and Image-guided Therapy, Medical University of Vienna, Vienna, Austria}
 \country{nan}
}

\author{Ying Peng}
\affiliation{%
 \institution{Shaanxi Normal University}
 \country{nan}
}

\author{Guiming Dong}
\affiliation{%
 \institution{University of Electronic Science and Technology of China}
 \country{nan}
}

\author{Moona Mazher}
\affiliation{%
 \institution{PhD student}
 \country{nan}
}

\author{Helena Torres}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Mireia Alenyà}
\affiliation{%
 \institution{BCN-MedTech, Department of Information and Communications Technologies, Universitat Pompeu Fabra}
 \country{nan}
}

\author{Lin Yang}
\affiliation{%
 \institution{hkust}
 \country{nan}
}

\author{ZunHyan (Clarence) Rieu}
\affiliation{%
 \institution{NEUROPHET Research Institute}
 \country{nan}
}

\author{KuanLun Liao}
\affiliation{%
 \institution{Real Doctor AI Research Centre}
 \country{nan}
}

\author{Fereshteh Yousefirizi}
\affiliation{%
 \institution{Post-doctoral researcher, BC Cancer research Institute}
 \country{nan}
}

\author{mehdi fatan serj}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Tao Liu}
\affiliation{%
 \institution{Jiangnan University}
 \country{nan}
}

\author{Gowtham Krishnan Murugesan}
\affiliation{%
 \institution{BAMF Health}
 \country{nan}
}

\author{Daniel Lang}
\affiliation{%
 \institution{Helmholtz Zentrum München, Institute of Radiation Medicine; Technical University of Munich, Physics Department}
 \country{nan}
}

\author{Mingyuan Meng}
\affiliation{%
 \institution{The University of Sydney}
 \country{nan}
}

\author{Numan Saeed}
\affiliation{%
 \institution{Mohamed Bin Zayed University of Science and Technology}
 \country{nan}
}

\author{Mohamed Naser}
\affiliation{%
 \institution{MD Anderson Cancer Center}
 \country{nan}
}

\author{Kareem A. Wahid}
\affiliation{%
 \institution{MD Anderson Cancer Center}
 \country{nan}
}

\author{Jintao Ren}
\affiliation{%
 \institution{Aarhus University}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{postdoc researcher}
 \country{nan}
}

\author{Jiangshan Lu}
\affiliation{%
 \institution{University of Electronic Science and Technology of China}
 \country{nan}
}

\author{Chengyang An}
\affiliation{%
 \institution{Shanghai Jiao Tong University, Shanghai, China}
 \country{nan}
}

\author{Ryan Gifford}
\affiliation{%
 \institution{Ohio State University}
 \country{nan}
}

\author{Minjeong Cho}
\affiliation{%
 \institution{Chung-Ang University}
 \country{nan}
}

\author{Sebastian Starke}
\affiliation{%
 \institution{Helmholtz-Zentrum Dresden-Rossendorf}
 \country{nan}
}

\author{Angel Victor Juanco Muller}
\affiliation{%
 \institution{Heriot-Watt University; Canon Medical Research Europe}
 \country{nan}
}

\author{Luyi Han}
\affiliation{%
 \institution{NKI}
 \country{nan}
}

\author{Marek Wodzinski}
\affiliation{%
 \institution{AGH UST, Department of Measurement and Electronics}
 \country{nan}
}

\author{Tony Chi Wing Mok}
\affiliation{%
 \institution{The Hong Kong University of Science and Technology}
 \country{nan}
}

\author{Bailiang Jian}
\affiliation{%
 \institution{Technical University of Munich}
 \country{nan}
}

\author{Mikael Brudfors}
\affiliation{%
 \institution{Wellcome Centre for Human Neuroimaging, University College London, London, UK}
 \country{nan}
}

\author{Wei Shao}
\affiliation{%
 \institution{Department of Radiology, Stanford University}
 \country{nan}
}

\author{Daniel Grzech}
\affiliation{%
 \institution{Imperial College London}
 \country{nan}
}

\author{Wentao Pan}
\affiliation{%
 \institution{Tsinghua Shenzhen International Graduate School}
 \country{nan}
}

\author{Hanqiu Deng}
\affiliation{%
 \institution{Department of Electrical and Computer Engineering, University of Alberta}
 \country{nan}
}

\author{Felix Meissen}
\affiliation{%
 \institution{Klinikum rechts der Isar of the Technical University of Munich}
 \country{nan}
}

\author{Jeremy Tan}
\affiliation{%
 \institution{Imperial College London}
 \country{nan}
}

\author{Lars Doorenbos}
\affiliation{%
 \institution{University of Bern}
 \country{nan}
}

\author{Inha Kang}
\affiliation{%
 \institution{Korea Advanced Institute of Science and Technology}
 \country{nan}
}

\author{Florentin Bieder}
\affiliation{%
 \institution{University of Basel}
 \country{nan}
}

\author{Ramin Nateghi}
\affiliation{%
 \institution{Shiraz University of Technology}
 \country{nan}
}

\author{Seyed Hossein Mirjahanmardi}
\affiliation{%
 \institution{Postdoctorate Fellow, Ryerson University}
 \country{nan}
}

\author{salar razavi}
\affiliation{%
 \institution{Ryerson University}
 \country{nan}
}

\author{Mustaffa Hussain}
\affiliation{%
 \institution{Onward Assist}
 \country{nan}
}

\author{Jack Breen}
\affiliation{%
 \institution{University of Leeds}
 \country{nan}
}

\author{Satoshi Kondo}
\affiliation{%
 \institution{Muroran Institute of Technology}
 \country{nan}
}

\author{Markus Huellebrand}
\affiliation{%
 \institution{Charité - Universitätsmedizin Berlin}
 \country{nan}
}

\author{Sandro Queirós}
\affiliation{%
 \institution{Life and Health Sciences Research Institute (ICVS), School of Medicine, University of Minho, Braga, Portugal; ICVS/3B’s - PT Government Associate Laboratory, Braga/Guimarães, Portugal}
 \country{nan}
}

\author{Kumaradevan Punithakumar}
\affiliation{%
 \institution{University of Alberta}
 \country{nan}
}

\author{Moona Mazher}
\affiliation{%
 \institution{Department of Computer Engineering and Mathematics, University Rovira i Virgili, Spain}
 \country{nan}
}

\author{Tewodros Weldebirhan AREGA}
\affiliation{%
 \institution{ImViA Laboratory, Université Bourgogne Franche-Comté, Dijon, France}
 \country{nan}
}

\author{Christoforos Galazis}
\affiliation{%
 \institution{Department of Computing, Imperial College London and National Heart and Lung Institute, Imperial College London}
 \country{nan}
}

\author{Zheyao Gao}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Francesco Galati}
\affiliation{%
 \institution{EURECOM}
 \country{nan}
}

\author{Hassan Mohy-ud-Din}
\affiliation{%
 \institution{LUMS School of Science and Engineering, Lahore, Pakistan}
 \country{nan}
}

\author{Xiaowu Sun}
\affiliation{%
 \institution{Leiden University Medica Center}
 \country{nan}
}

\author{Mitchell Fulton}
\affiliation{%
 \institution{University of Colorado, Boulder}
 \country{nan}
}

\author{Di Liu}
\affiliation{%
 \institution{Rutgers University}
 \country{nan}
}

\author{Yasmina Al Khalil}
\affiliation{%
 \institution{Eindhoven University of Technology, Eindhoven, The Netherlands}
 \country{nan}
}

\author{Jorge Corral Acero}
\affiliation{%
 \institution{University of Oxford}
 \country{nan}
}

\author{Marcel Beetz}
\affiliation{%
 \institution{University of Oxford}
 \country{nan}
}

\author{Shengbo Gao}
\affiliation{%
 \institution{Beihang University}
 \country{nan}
}

\author{Jimut Bahan Pal}
\affiliation{%
 \institution{Ramakrishna Mission Vivekananda Educational and Research Institute}
 \country{nan}
}

\author{João Lourenço Silva}
\affiliation{%
 \institution{INESC-ID / Instituto Superior Técnico, University of Lisbon}
 \country{nan}
}

\author{Yucong Chen}
\affiliation{%
 \institution{ShanghaiTech University}
 \country{nan}
}

\author{Yingbin Bai}
\affiliation{%
 \institution{The University of Sydney }
 \country{nan}
}

\author{Anindo Saha}
\affiliation{%
 \institution{PhD Candidate, Diagnostic Image Analysis Group, Radboud University Medical Center}
 \country{nan}
}

\author{Wei Wang}
\affiliation{%
 \institution{Southern University of Science and Technology}
 \country{nan}
}

\author{Xiong Wang}
\affiliation{%
 \institution{OPPO Research Institute}
 \country{nan}
}

\author{Jiachen ZHAO}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Pengcheng Shi}
\affiliation{%
 \institution{Harbin Institute of Technology, Shenzhen}
 \country{nan}
}

\author{Mina Rezaei}
\affiliation{%
 \institution{LMU Munich}
 \country{nan}
}

\author{Dewen Zeng}
\affiliation{%
 \institution{University of Notre Dame}
 \country{nan}
}

\author{Timothy Sum Hon Mun}
\affiliation{%
 \institution{Institute of Cancer Research}
 \country{nan}
}

\author{Stephan Huschauer}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Ramy Ashraf Zeineldin}
\affiliation{%
 \institution{Health Robotics and Automation (HERA), Karlsruhe Institute of Technology, Germany; Research Group Computer Assisted Medicine (CaMed), Reutlingen University, Germany; Faculty of Electronic Engineering (FEE), Menoufia University, Egypt}
 \country{nan}
}

\author{Johannes Roth}
\affiliation{%
 \institution{Leipzig University}
 \country{nan}
}

\author{Jakub Nalepa}
\affiliation{%
 \institution{Silesian University of Technology, Gliwice, Poland; Future Processing Healthcare, Gliwice, Poland}
 \country{nan}
}

\author{Zhifan Jiang}
\affiliation{%
 \institution{Sheikh Zayed Institute for Pediatric Surgical Innovation, Children's National Hospital; NVIDIA}
 \country{nan}
}

\author{IL SONG HAN}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Ning Wen}
\affiliation{%
 \institution{Henry Ford Health System}
 \country{nan}
}

\author{Ali Hatamizadeh}
\affiliation{%
 \institution{NVIDIA}
 \country{nan}
}

\author{Timothy Sum Hon Mun}
\affiliation{%
 \institution{Institute of Cancer Research}
 \country{nan}
}

\author{Huan Minh Luu}
\affiliation{%
 \institution{MRI Lab, Department of Bio and Brain Engineering, Korea Advanced Institute of Science and Technology}
 \country{nan}
}

\author{Kamlesh Pawar}
\affiliation{%
 \institution{Monash University}
 \country{nan}
}

\author{Daniel Chen}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Tomoo Inubushi}
\affiliation{%
 \institution{Hamamatsu Photonics K.K.}
 \country{nan}
}

\author{Jonathan Adam Rico}
\affiliation{%
 \institution{University of San Agustin, Center for Informatics, Iloilo City, Philippines}
 \country{nan}
}

\author{SeongHun Jeong}
\affiliation{%
 \institution{KT}
 \country{nan}
}

\author{Qingshuo ZHENG}
\affiliation{%
 \institution{Surgical Robot Vision Group, Wellcome/EPSRC Centre for Interventional and Surgical Sciences(WEISS) and Department of Computer Science, University College London, London, UK}
 \country{nan}
}

\author{Lei Yu}
\affiliation{%
 \institution{Graz University of technology}
 \country{nan}
}

\author{Xingyu Li}
\affiliation{%
 \institution{University of Alberta}
 \country{nan}
}

\author{Jianning Li}
\affiliation{%
 \institution{Graz University of Technology  \&  University Hospital Essen}
 \country{nan}
}

\author{Artem Kroviakov}
\affiliation{%
 \institution{Institute of Computer Graphics and Vision, Graz University of Technology}
 \country{nan}
}

\author{Hugo Kuijf}
\affiliation{%
 \institution{UMC Utrecht}
 \country{nan}
}

\author{Minho Lee}
\affiliation{%
 \institution{Neurophet Inc.}
 \country{nan}
}

\author{Pengcheng Shi}
\affiliation{%
 \institution{Harbin Institute of Technology, Shenzhen}
 \country{nan}
}

\author{Heonjin Ha}
\affiliation{%
 \institution{nan}
 \country{nan}
}

\author{Chunxu Guo}
\affiliation{%
 \institution{ShanghaiTech University School of Biomedical Engineering IDEALab}
 \country{nan}
}

\author{Abdul Qayyum}
\affiliation{%
 \institution{postdoc researcher}
 \country{nan}
}

\author{Amirreza Mahbod}
\affiliation{%
 \institution{Medical University of Vienna}
 \country{nan}
}

\author{Richard McKinley}
\affiliation{%
 \institution{Support Centre for Advanced Neuroimaging, University institute for diagnostic and interventional neuroradiology, university hospital Bern}
 \country{nan}
}

\author{Uzay Macar}
\affiliation{%
 \institution{1. NeuroPoly Lab, Institute of Biomedical Engineering, Polytechnique Montréal, Montréal, QC, Canada; 2. MILA - Québec AI Institute, Montréal, QC, Canada}
 \country{nan}
}

\author{Julien Cohen-Adad}
\affiliation{%
 \institution{1. NeuroPoly Lab, Institute of Biomedical Engineering, Polytechnique Montréal, Montréal, QC, Canada; 2. MILA - Québec AI Institute, Montréal, QC, Canada}
 \country{nan}
}

\author{Mariano Cabezas}
\affiliation{%
 \institution{Brain and Mind Centre, The University of Sydney}
 \country{nan}
}

\author{Julia Andresen}
\affiliation{%
 \institution{University of Lübeck, Institute of Medical Informatics}
 \country{nan}
}

\author{Domen Preložnik}
\affiliation{%
 \institution{Laboratory of Imaging Technologies - Faculty of Electrical Engineering, University of Ljubljana}
 \country{nan}
}

\author{Reda Abdellah KAMRAOUI}
\affiliation{%
 \institution{Université de Bordeaux}
 \country{nan}
}

\author{Alexandre FENNETEAU}
\affiliation{%
 \institution{XLIM Laboratory, University of Poitiers, UMR CNRS 7252 - Poitiers, France; I3M, Common Laboratory CNRS-Siemens - University and Hospital of Poitiers ; Poitiers, France - Neuroimaging Department, Quinze Vingts Hospital; Paris, France; Siemens Healthcare, Saint Denis, France}
 \country{nan}
}

\author{Francesco La Rosa}
\affiliation{%
 \institution{LTS5, Ecole Polytechnique Fédérale de Lausanne, Switzerland.}
 \country{nan}
}

\author{Adam Gibicar}
\affiliation{%
 \institution{Ryerson University}
 \country{nan}
}

\author{Samir Mitha}
\affiliation{%
 \institution{Department of Electrical, Computer and Biomedical Engineering, Ryerson University, Toronto, ON, Canada}
 \country{nan}
}

\author{April Khademi}
\affiliation{%
 \institution{Image Analysis in Medicine Lab (IAMLAB), Department of Electrical, Computer, and Biomedical Engineering, Ryerson University, Toronto, Canada; Keenan Research Center for Biomedical Science, St. Michael's Hospital, Unity Health Network, Toronto, Canada; Institute for Biomedical Engineering, Science, and Technology (iBEST), A Partnership Between St. Michael's Hospital and Ryerson University, Toronto, Canada}
 \country{nan}
}

\author{Ferran Prados Carrasco}
\affiliation{%
 \institution{CMIC - University College London and e-Health Center - Universitat Oberta de Catalunya}
 \country{nan}
}

\author{Mostafa Salem}
\affiliation{%
 \institution{Institute of Computer Vision and Robotics, University of Girona, Girona, Spain}
 \country{nan}
}

\author{Cory Efird}
\affiliation{%
 \institution{MacEwan University, Canada; University of Alberta, Canada}
 \country{nan}
}

\author{Dylan Miller}
\affiliation{%
 \institution{MacEwan University, Canada; University of Alberta, Canada}
 \country{nan}
}

\author{Dana Cobzas}
\affiliation{%
 \institution{MacEwan University, Canada; University of Alberta, Canada}
 \country{nan}
}

\author{Junghwa Kang}
\affiliation{%
 \institution{Hankuk University of Foreign Studies}
 \country{nan}
}

\author{Sebastian Hitziger}
\affiliation{%
 \institution{Mediaire}
 \country{nan}
}

\author{Théodore Soulier}
\affiliation{%
 \institution{Paris Brain Institute}
 \country{nan}
}

\author{Marcela de Oliveira}
\affiliation{%
 \institution{São Paulo State University (UNESP) - Brazil}
 \country{nan}
}

\author{Berke Doga Basaran}
\affiliation{%
 \institution{Department of Computing, Imperial College London}
 \country{nan}
}

\author{Huahong Zhang}
\affiliation{%
 \institution{Vanderbilt University}
 \country{nan}
}

\author{Brennan Nichyporuk}
\affiliation{%
 \institution{McGill University}
 \country{nan}
}

\author{Hwanseung Yoo}
\affiliation{%
 \institution{Hankuk University of Foreign Studies}
 \country{nan}
}

\author{hao bian}
\affiliation{%
 \institution{Tsinghua University}
 \country{nan}
}

\author{Kwang-Ju Kim}
\affiliation{%
 \institution{Electronics and Telecommunications Research Institute}
 \country{nan}
}

\author{chang hee gan}
\affiliation{%
 \institution{sejong university /korea university}
 \country{nan}
}

\author{Ramin Nateghi}
\affiliation{%
 \institution{Department of Electrical and Electronics Engineering, Shiraz University of Technology, Shiraz, Iran}
 \country{nan}
}

\author{Fattaneh Pourakpour}
\affiliation{%
 \institution{Iranian Brain Mapping Biobank(IBMB), National Brain Mapping Laboratory (NBML), Tehran, Iran}
 \country{nan}
}

\author{Yanling Liu}
\affiliation{%
 \institution{Leidos Biomed.}
 \country{nan}
}

\author{Amirsaeed Yazdani}
\affiliation{%
 \institution{The Pennsylvania State university}
 \country{nan}
}

\author{Caroline Petitjean}
\affiliation{%
 \institution{Université de Rouen Normandie}
 \country{France}
}

\author{Daniel Sage}
\affiliation{%
 \institution{EPFL}
 \country{Switzerland}
}

\author{Jan Kybic}
\affiliation{%
 \institution{Czech Technical University}
 \country{Czech Republic}
}

\author{Anne Martel}
\affiliation{%
 \institution{Department of Medical Biophysics, University of Toronto, Ontario, Canada; Physical Sciences, Sunnybrook Research Institute, Toronto, Ontario}
 \country{Canada}
}

\author{Bennett Landman}
\affiliation{%
 \institution{Electrical Engineering, Vanderbilt University, Nashville, Tennessee}
 \country{USA}
}



==> tables/data_explored_vs_used.tex <==
\begin{longtable}{ p{7cm} p{3cm} p{3cm} }
\label{tab:data_exploration_vs_usage} \\
\caption{\textcolor{red}{Comparison of different types of additional data (i.e. data not provided for the respective competition) that was explored by all respondents and used in the DL-based solutions. In this context, “exploring” also means analyzing data that was incorporated in the final solution. The respondents were allowed to pick multiple answers.}} \\
\toprule
Type of data & Exploration of additional data (n = 42) & Usage of additional data in final solution (n = 20) \\* \midrule
\endfirsthead
%
\multicolumn{2}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Type of data & Percentage of respondents (n = 42) exploring additional data & Percentage of respondents (n = 20) using additional data in final solution \\* \midrule
\endhead
%
Biomedical data for same type of task - public & 48\% & 40\% \\
Biomedical data for same type of task - private & 36\% & 25\% \\
Biomedical data for different type of task - public & 21\% & 15\% \\
Biomedical data for different type of task - private & 10\% & 0\% \\
Non-biomedical data - public & 7\% & 5\% \\
Non-biomedical data - private & 0\% & 0\% \\
Re-annotated data & 2\% & 0\% \\* \bottomrule
\end{longtable}

==> tables/dl_aspects.tex <==
\begin{longtable}{ p{10cm} p{3cm} }
\label{tab:dl_aspects} \\
\caption{\textcolor{red}{Aspects that respondents who submitted a DL-based solution spent most time on. The respondents were allowed to pick up to three answers.}} \\
\toprule
Aspect & Percentage of respondents (n = 233) \\* \midrule
\endfirsthead
%
\multicolumn{2}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Aspect & Percentage of respondents (n = 233) \\* \midrule
\endhead
%
Selecting one or multiple existing architectures (e.g., U-Net, ResNet, DenseNet) that best match the task & 45\% \\
Configuring the data augmentation & 33\% \\
Configuring the template architecture (e.g., How deep? How many stages/pooling layers?) & 28\% \\
Exploring existing loss functions & 25\% \\
Ensembling & 22\% \\
Choosing a template architecture & 17\% \\
Other new methodological contributions (besides architecture; e.g., task-specific loss) & 16\% \\
Optimizing postprocessing (e.g., aggregating predictions during inference) & 15\% \\* \bottomrule
\end{longtable}
